Nuclear Physics under the low-energy, high intensity frontier

Despite numerous achievements and recent progress, nuclear physics is often (wrongly) considered an old field of research nowadays. However, developments in theoretical frameworks and reliable experimental techniques have made the field mature enough to explore many new frontiers. In this regard, extending existing knowledge to an emerging field of physics -- where particles interact with a relatively low-energy but high intensity field (intense enough so that multi-particle processes become comparable or more important than one-to-one processes) -- can lead to exciting discoveries. Investigations can be realized under a highly time-compressed beam source (e.g., particle sources generated by laser-matter interaction using high-power laser systems). Here we focus on a new scheme, where high-power laser systems are exploited as a driver to generate energetic ($\gamma$-ray) photons. Together with additional low-energy photons provided by a second, less intense laser, a multi-photon absorption scheme enables a very attainable manipulation of nuclear transitions including isomer pumping and depletion.

==> gammaplot_f <==
# Grace project file
#
@version 50125
@page size 792, 612
@page scroll 5%
@page inout 5%
@link page off
@map font 8 to "Courier", "Courier"
@map font 10 to "Courier-Bold", "Courier-Bold"
@map font 14 to "Courier-BoldItalic", "Courier-BoldItalic"
@map font 11 to "Courier-BoldOblique", "Courier-BoldOblique"
@map font 16 to "Courier-Italic", "Courier-Italic"
@map font 9 to "Courier-Oblique", "Courier-Oblique"
@map font 18 to "Courier-Regular", "Courier-Regular"
@map font 19 to "D050000L-Regular", "D050000L-Regular"
@map font 4 to "Helvetica", "Helvetica"
@map font 6 to "Helvetica-Bold", "Helvetica-Bold"
@map font 7 to "Helvetica-BoldOblique", "Helvetica-BoldOblique"
@map font 5 to "Helvetica-Oblique", "Helvetica-Oblique"
@map font 29 to "NimbusMonoPS-Bold", "NimbusMonoPS-Bold"
@map font 30 to "NimbusMonoPS-BoldItalic", "NimbusMonoPS-BoldItalic"
@map font 31 to "NimbusMonoPS-Italic", "NimbusMonoPS-Italic"
@map font 32 to "NimbusMonoPS-Regular", "NimbusMonoPS-Regular"
@map font 33 to "NimbusRoman-Bold", "NimbusRoman-Bold"
@map font 34 to "NimbusRoman-BoldItalic", "NimbusRoman-BoldItalic"
@map font 35 to "NimbusRoman-Italic", "NimbusRoman-Italic"
@map font 36 to "NimbusRoman-Regular", "NimbusRoman-Regular"
@map font 41 to "NimbusSans-Bold", "NimbusSans-Bold"
@map font 42 to "NimbusSans-BoldItalic", "NimbusSans-BoldItalic"
@map font 43 to "NimbusSans-Italic", "NimbusSans-Italic"
@map font 44 to "NimbusSans-Regular", "NimbusSans-Regular"
@map font 53 to "NimbusSansNarrow-Bold", "NimbusSansNarrow-Bold"
@map font 54 to "NimbusSansNarrow-BoldOblique", "NimbusSansNarrow-BoldOblique"
@map font 55 to "NimbusSansNarrow-Oblique", "NimbusSansNarrow-Oblique"
@map font 56 to "NimbusSansNarrow-Regular", "NimbusSansNarrow-Regular"
@map font 57 to "P052-Bold", "P052-Bold"
@map font 58 to "P052-BoldItalic", "P052-BoldItalic"
@map font 59 to "P052-Italic", "P052-Italic"
@map font 60 to "P052-Roman", "P052-Roman"
@map font 62 to "StandardSymbolsPS-Regular", "StandardSymbolsPS-Regular"
@map font 12 to "Symbol", "Symbol"
@map font 2 to "Times-Bold", "Times-Bold"
@map font 3 to "Times-BoldItalic", "Times-BoldItalic"
@map font 1 to "Times-Italic", "Times-Italic"
@map font 0 to "Times-Roman", "Times-Roman"
@map font 68 to "URWBookman-Demi", "URWBookman-Demi"
@map font 69 to "URWBookman-DemiItalic", "URWBookman-DemiItalic"
@map font 70 to "URWBookman-Light", "URWBookman-Light"
@map font 71 to "URWBookman-LightItalic", "URWBookman-LightItalic"
@map font 77 to "URWGothic-Book", "URWGothic-Book"
@map font 78 to "URWGothic-BookOblique", "URWGothic-BookOblique"
@map font 79 to "URWGothic-Demi", "URWGothic-Demi"
@map font 80 to "URWGothic-DemiOblique", "URWGothic-DemiOblique"
@map font 89 to "Utopia-Bold", "Utopia-Bold"
@map font 90 to "Utopia-BoldItalic", "Utopia-BoldItalic"
@map font 91 to "Utopia-Italic", "Utopia-Italic"
@map font 92 to "Utopia-Regular", "Utopia-Regular"
@map font 93 to "Z003-MediumItalic", "Z003-MediumItalic"
@map font 13 to "ZapfDingbats", "ZapfDingbats"
@map color 0 to (255, 255, 255), "white"
@map color 1 to (0, 0, 0), "black"
@map color 2 to (255, 0, 0), "red"
@map color 3 to (0, 255, 0), "green"
@map color 4 to (0, 0, 255), "blue"
@map color 5 to (255, 255, 0), "yellow"
@map color 6 to (188, 143, 143), "brown"
@map color 7 to (220, 220, 220), "grey"
@map color 8 to (148, 0, 211), "violet"
@map color 9 to (0, 255, 255), "cyan"
@map color 10 to (255, 0, 255), "magenta"
@map color 11 to (255, 165, 0), "orange"
@map color 12 to (114, 33, 188), "indigo"
@map color 13 to (103, 7, 72), "maroon"
@map color 14 to (64, 224, 208), "turquoise"
@map color 15 to (0, 139, 0), "green4"
@reference date 0
@date wrap off
@date wrap year 1950
@default linewidth 1.0
@default linestyle 1
@default color 1
@default pattern 1
@default font 0
@default char size 1.000000
@default symbol size 1.000000
@default sformat "%.8g"
@background color 0
@page background fill on
@timestamp off
@timestamp 0.03, 0.03
@timestamp color 1
@timestamp rot 0
@timestamp font 0
@timestamp char size 1.000000
@timestamp def "Mon Feb  3 15:55:24 2025"
@with line
@    line on
@    line loctype view
@    line 0.175, 0.36887254902, 0.185, 0.36887254902
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.175, 0.34681372549, 0.185, 0.34681372549
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.175, 0.270833333333, 0.185, 0.270833333333
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.186274509804, 0.367647058824, 0.186274509804, 0.269607843137
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.186274509804, 0.269607843137, 0.1875, 0.269607843137
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.186274509804, 0.322303921569, 0.232843137255, 0.289215686275
@    line linewidth 1.0
@    line linestyle 1
@    line color 1
@    line arrow 0
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with line
@    line on
@    line loctype view
@    line 0.223039215686, 0.296568627451, 0.227941176471, 0.292892156863
@    line linewidth 2.0
@    line linestyle 1
@    line color 1
@    line arrow 2
@    line arrow type 0
@    line arrow length 1.000000
@    line arrow layout 1.000000, 1.000000
@line def
@with string
@    string on
@    string loctype view
@    string 0.21401960784, 0.248382352941
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.500000
@    string def "At 1 MeV"
@with string
@    string on
@    string loctype view
@    string 0.7, 0.25
@    string color 1
@    string rot 0
@    string font 0
@    string just 0
@    string char size 1.500000
@    string def "At 58 MeV"
@r0 off
@link r0 to g0
@r0 type above
@r0 linestyle 1
@r0 linewidth 1.0
@r0 color 1
@r0 line 0, 0, 0, 0
@r1 off
@link r1 to g0
@r1 type above
@r1 linestyle 1
@r1 linewidth 1.0
@r1 color 1
@r1 line 0, 0, 0, 0
@r2 off
@link r2 to g0
@r2 type above
@r2 linestyle 1
@r2 linewidth 1.0
@r2 color 1
@r2 line 0, 0, 0, 0
@r3 off
@link r3 to g0
@r3 type above
@r3 linestyle 1
@r3 linewidth 1.0
@r3 color 1
@r3 line 0, 0, 0, 0
@r4 off
@link r4 to g0
@r4 type above
@r4 linestyle 1
@r4 linewidth 1.0
@r4 color 1
@r4 line 0, 0, 0, 0
@g0 on
@g0 hidden false
@g0 type XY
@g0 stacked false
@g0 bar hgap 0.000000
@g0 fixedpoint off
@g0 fixedpoint type 0
@g0 fixedpoint xy 0.000000, 0.000000
@g0 fixedpoint format general general
@g0 fixedpoint prec 6, 6
@with g0
@    world 0, 9.5, 100, 15
@    stack world 0, 0, 0, 0
@    znorm 1
@    view 0.150000, 0.150000, 1.244118, 0.500000
@    title ""
@    title font 0
@    title size 1.500000
@    title color 1
@    subtitle ""
@    subtitle font 0
@    subtitle size 1.000000
@    subtitle color 1
@    xaxes scale Normal
@    yaxes scale Normal
@    xaxes invert off
@    yaxes invert off
@    xaxis  on
@    xaxis  type zero false
@    xaxis  offset 0.000000 , 0.000000
@    xaxis  bar on
@    xaxis  bar color 1
@    xaxis  bar linestyle 1
@    xaxis  bar linewidth 1.0
@    xaxis  label "E\s\xg\0\N (MeV)"
@    xaxis  label layout para
@    xaxis  label place auto
@    xaxis  label char size 1.750000
@    xaxis  label font 0
@    xaxis  label color 1
@    xaxis  label place normal
@    xaxis  tick on
@    xaxis  tick major 20
@    xaxis  tick minor ticks 1
@    xaxis  tick default 6
@    xaxis  tick place rounded true
@    xaxis  tick in
@    xaxis  tick major size 1.000000
@    xaxis  tick major color 1
@    xaxis  tick major linewidth 1.0
@    xaxis  tick major linestyle 1
@    xaxis  tick major grid off
@    xaxis  tick minor color 1
@    xaxis  tick minor linewidth 1.0
@    xaxis  tick minor linestyle 1
@    xaxis  tick minor grid off
@    xaxis  tick minor size 0.500000
@    xaxis  ticklabel on
@    xaxis  ticklabel format general
@    xaxis  ticklabel prec 5
@    xaxis  ticklabel formula ""
@    xaxis  ticklabel append ""
@    xaxis  ticklabel prepend ""
@    xaxis  ticklabel angle 0
@    xaxis  ticklabel skip 0
@    xaxis  ticklabel stagger 0
@    xaxis  ticklabel place normal
@    xaxis  ticklabel offset auto
@    xaxis  ticklabel offset 0.000000 , 0.010000
@    xaxis  ticklabel start type auto
@    xaxis  ticklabel start 0.000000
@    xaxis  ticklabel stop type auto
@    xaxis  ticklabel stop 0.000000
@    xaxis  ticklabel char size 1.750000
@    xaxis  ticklabel font 0
@    xaxis  ticklabel color 1
@    xaxis  tick place both
@    xaxis  tick spec type none
@    yaxis  on
@    yaxis  type zero false
@    yaxis  offset 0.000000 , 0.000000
@    yaxis  bar on
@    yaxis  bar color 1
@    yaxis  bar linestyle 1
@    yaxis  bar linewidth 1.0
@    yaxis  label "Log\s10\N(N\s\xg\0\N)(eV\S-1\Ncm\S-2\N)"
@    yaxis  label layout para
@    yaxis  label place auto
@    yaxis  label char size 1.750000
@    yaxis  label font 0
@    yaxis  label color 1
@    yaxis  label place normal
@    yaxis  tick on
@    yaxis  tick major 1
@    yaxis  tick minor ticks 1
@    yaxis  tick default 6
@    yaxis  tick place rounded true
@    yaxis  tick in
@    yaxis  tick major size 1.000000
@    yaxis  tick major color 1
@    yaxis  tick major linewidth 1.0
@    yaxis  tick major linestyle 1
@    yaxis  tick major grid off
@    yaxis  tick minor color 1
@    yaxis  tick minor linewidth 1.0
@    yaxis  tick minor linestyle 1
@    yaxis  tick minor grid off
@    yaxis  tick minor size 0.500000
@    yaxis  ticklabel on
@    yaxis  ticklabel format general
@    yaxis  ticklabel prec 5
@    yaxis  ticklabel formula ""
@    yaxis  ticklabel append ""
@    yaxis  ticklabel prepend ""
@    yaxis  ticklabel angle 0
@    yaxis  ticklabel skip 0
@    yaxis  ticklabel stagger 0
@    yaxis  ticklabel place normal
@    yaxis  ticklabel offset auto
@    yaxis  ticklabel offset 0.000000 , 0.010000
@    yaxis  ticklabel start type auto
@    yaxis  ticklabel start 0.000000
@    yaxis  ticklabel stop type auto
@    yaxis  ticklabel stop 0.000000
@    yaxis  ticklabel char size 1.750000
@    yaxis  ticklabel font 0
@    yaxis  ticklabel color 1
@    yaxis  tick place both
@    yaxis  tick spec type none
@    altxaxis  off
@    altyaxis  off
@    legend on
@    legend loctype view
@    legend 0.95, 0.47
@    legend box color 1
@    legend box pattern 1
@    legend box linewidth 1.0
@    legend box linestyle 1
@    legend box fill color 0
@    legend box fill pattern 1
@    legend font 0
@    legend char size 1.750000
@    legend color 1
@    legend length 4
@    legend vgap 1
@    legend hgap 1
@    legend invert false
@    frame type 0
@    frame linestyle 1
@    frame linewidth 1.0
@    frame color 1
@    frame pattern 1
@    frame background color 0
@    frame background pattern 0
@    s0 hidden false
@    s0 type xy
@    s0 symbol 0
@    s0 symbol size 1.000000
@    s0 symbol color 1
@    s0 symbol pattern 1
@    s0 symbol fill color 1
@    s0 symbol fill pattern 0
@    s0 symbol linewidth 1.0
@    s0 symbol linestyle 1
@    s0 symbol char 65
@    s0 symbol char font 0
@    s0 symbol skip 0
@    s0 line type 1
@    s0 line linestyle 1
@    s0 line linewidth 2.5
@    s0 line color 1
@    s0 line pattern 1
@    s0 baseline type 0
@    s0 baseline off
@    s0 dropline off
@    s0 fill type 0
@    s0 fill rule 0
@    s0 fill color 1
@    s0 fill pattern 1
@    s0 avalue off
@    s0 avalue type 2
@    s0 avalue char size 1.000000
@    s0 avalue font 0
@    s0 avalue color 1
@    s0 avalue rot 0
@    s0 avalue format general
@    s0 avalue prec 3
@    s0 avalue prepend ""
@    s0 avalue append ""
@    s0 avalue offset 0.000000 , 0.000000
@    s0 errorbar on
@    s0 errorbar place both
@    s0 errorbar color 1
@    s0 errorbar pattern 1
@    s0 errorbar size 1.000000
@    s0 errorbar linewidth 1.0
@    s0 errorbar linestyle 1
@    s0 errorbar riser linewidth 1.0
@    s0 errorbar riser linestyle 1
@    s0 errorbar riser clip off
@    s0 errorbar riser clip length 0.100000
@    s0 comment "/home/chiehjen/Downloads/fort.11"
@    s0 legend  "Ref. [5]"
@    s1 hidden false
@    s1 type xy
@    s1 symbol 2
@    s1 symbol size 1.000000
@    s1 symbol color 11
@    s1 symbol pattern 1
@    s1 symbol fill color 11
@    s1 symbol fill pattern 1
@    s1 symbol linewidth 1.0
@    s1 symbol linestyle 1
@    s1 symbol char 65
@    s1 symbol char font 0
@    s1 symbol skip 0
@    s1 line type 0
@    s1 line linestyle 1
@    s1 line linewidth 1.0
@    s1 line color 11
@    s1 line pattern 1
@    s1 baseline type 0
@    s1 baseline off
@    s1 dropline off
@    s1 fill type 0
@    s1 fill rule 0
@    s1 fill color 1
@    s1 fill pattern 1
@    s1 avalue off
@    s1 avalue type 2
@    s1 avalue char size 1.000000
@    s1 avalue font 0
@    s1 avalue color 1
@    s1 avalue rot 0
@    s1 avalue format general
@    s1 avalue prec 3
@    s1 avalue prepend ""
@    s1 avalue append ""
@    s1 avalue offset 0.000000 , 0.000000
@    s1 errorbar on
@    s1 errorbar place both
@    s1 errorbar color 11
@    s1 errorbar pattern 1
@    s1 errorbar size 1.000000
@    s1 errorbar linewidth 1.0
@    s1 errorbar linestyle 1
@    s1 errorbar riser linewidth 1.0
@    s1 errorbar riser linestyle 1
@    s1 errorbar riser clip off
@    s1 errorbar riser clip length 0.100000
@    s1 comment "/home/chiehjen/Downloads/4"
@    s1 legend  "Ref. [6]"
@    s2 hidden false
@    s2 type xy
@    s2 symbol 3
@    s2 symbol size 1.000000
@    s2 symbol color 2
@    s2 symbol pattern 1
@    s2 symbol fill color 2
@    s2 symbol fill pattern 1
@    s2 symbol linewidth 1.0
@    s2 symbol linestyle 1
@    s2 symbol char 65
@    s2 symbol char font 0
@    s2 symbol skip 0
@    s2 line type 0
@    s2 line linestyle 1
@    s2 line linewidth 1.0
@    s2 line color 2
@    s2 line pattern 1
@    s2 baseline type 0
@    s2 baseline off
@    s2 dropline off
@    s2 fill type 0
@    s2 fill rule 0
@    s2 fill color 1
@    s2 fill pattern 1
@    s2 avalue off
@    s2 avalue type 2
@    s2 avalue char size 1.000000
@    s2 avalue font 0
@    s2 avalue color 1
@    s2 avalue rot 0
@    s2 avalue format general
@    s2 avalue prec 3
@    s2 avalue prepend ""
@    s2 avalue append ""
@    s2 avalue offset 0.000000 , 0.000000
@    s2 errorbar on
@    s2 errorbar place both
@    s2 errorbar color 2
@    s2 errorbar pattern 1
@    s2 errorbar size 1.000000
@    s2 errorbar linewidth 1.0
@    s2 errorbar linestyle 1
@    s2 errorbar riser linewidth 1.0
@    s2 errorbar riser linestyle 1
@    s2 errorbar riser clip off
@    s2 errorbar riser clip length 0.100000
@    s2 comment "/home/chiehjen/Downloads/1"
@    s2 legend  "Ref. [7]"
@    s3 hidden false
@    s3 type xy
@    s3 symbol 4
@    s3 symbol size 1.000000
@    s3 symbol color 3
@    s3 symbol pattern 1
@    s3 symbol fill color 3
@    s3 symbol fill pattern 1
@    s3 symbol linewidth 1.0
@    s3 symbol linestyle 1
@    s3 symbol char 65
@    s3 symbol char font 0
@    s3 symbol skip 0
@    s3 line type 0
@    s3 line linestyle 1
@    s3 line linewidth 1.0
@    s3 line color 3
@    s3 line pattern 1
@    s3 baseline type 0
@    s3 baseline off
@    s3 dropline off
@    s3 fill type 0
@    s3 fill rule 0
@    s3 fill color 1
@    s3 fill pattern 1
@    s3 avalue off
@    s3 avalue type 2
@    s3 avalue char size 1.000000
@    s3 avalue font 0
@    s3 avalue color 1
@    s3 avalue rot 0
@    s3 avalue format general
@    s3 avalue prec 3
@    s3 avalue prepend ""
@    s3 avalue append ""
@    s3 avalue offset 0.000000 , 0.000000
@    s3 errorbar on
@    s3 errorbar place both
@    s3 errorbar color 3
@    s3 errorbar pattern 1
@    s3 errorbar size 1.000000
@    s3 errorbar linewidth 1.0
@    s3 errorbar linestyle 1
@    s3 errorbar riser linewidth 1.0
@    s3 errorbar riser linestyle 1
@    s3 errorbar riser clip off
@    s3 errorbar riser clip length 0.100000
@    s3 comment "/home/chiehjen/Downloads/2"
@    s3 legend  "Ref. [8]"
@    s4 hidden false
@    s4 type xy
@    s4 symbol 1
@    s4 symbol size 1.000000
@    s4 symbol color 4
@    s4 symbol pattern 1
@    s4 symbol fill color 4
@    s4 symbol fill pattern 1
@    s4 symbol linewidth 1.0
@    s4 symbol linestyle 1
@    s4 symbol char 65
@    s4 symbol char font 0
@    s4 symbol skip 0
@    s4 line type 0
@    s4 line linestyle 1
@    s4 line linewidth 1.0
@    s4 line color 4
@    s4 line pattern 1
@    s4 baseline type 0
@    s4 baseline off
@    s4 dropline off
@    s4 fill type 0
@    s4 fill rule 0
@    s4 fill color 1
@    s4 fill pattern 1
@    s4 avalue off
@    s4 avalue type 2
@    s4 avalue char size 1.000000
@    s4 avalue font 0
@    s4 avalue color 1
@    s4 avalue rot 0
@    s4 avalue format general
@    s4 avalue prec 3
@    s4 avalue prepend ""
@    s4 avalue append ""
@    s4 avalue offset 0.000000 , 0.000000
@    s4 errorbar on
@    s4 errorbar place both
@    s4 errorbar color 4
@    s4 errorbar pattern 1
@    s4 errorbar size 1.000000
@    s4 errorbar linewidth 1.0
@    s4 errorbar linestyle 1
@    s4 errorbar riser linewidth 1.0
@    s4 errorbar riser linestyle 1
@    s4 errorbar riser clip off
@    s4 errorbar riser clip length 0.100000
@    s4 comment "/home/chiehjen/Downloads/3"
@    s4 legend  "Ref. [9]"
@target G0.S0
@type xy
1 14.599396
2 14.424775
3 14.255941
4 14.092705
5 13.934875
6 13.782276
7 13.634735
8 13.492083
9 13.354157
10 13.220803
11 13.091867
12 12.967205
13 12.846674
14 12.730137
15 12.617461
16 12.50852
17 12.403189
18 12.301348
19 12.202881
20 12.107678
21 12.015631
22 11.926633
23 11.840584
24 11.757387
25 11.676948
26 11.599173
27 11.523976
28 11.451271
29 11.380976
30 11.313009
31 11.247295
32 11.183759
33 11.122329
34 11.062933
35 11.005506
36 10.949983
37 10.896299
38 10.844394
39 10.794209
40 10.745687
41 10.698774
42 10.653415
43 10.609559
44 10.567156
45 10.526159
46 10.48652
47 10.448194
48 10.411139
49 10.375312
50 10.340671
51 10.30718
52 10.274797
53 10.243488
54 10.213217
55 10.183948
56 10.15565
57 10.128289
58 10.101835
59 10.076258
60 10.051528
61 10.027617
62 10.004499
63 9.9821472
64 9.960536
65 9.939641
66 9.9194384
67 9.8999052
68 9.8810196
69 9.8627596
70 9.8451052
71 9.8280354
72 9.8115311
73 9.7955742
74 9.7801456
75 9.7652283
76 9.7508059
77 9.7368603
78 9.7233782
79 9.7103414
80 9.6977377
81 9.6855516
82 9.673769
83 9.6623774
84 9.6513624
85 9.6407137
86 9.6304169
87 9.6204615
88 9.610836
89 9.6015291
90 9.5925312
91 9.5838318
92 9.5754194
93 9.5672875
94 9.5594235
95 9.5518208
96 9.5444698
97 9.537363
98 9.5304909
99 9.5238476
&
@target G0.S1
@type xy
58 10.4
&
@target G0.S2
@type xy
1 12.6
&
@target G0.S3
@type xy
1 12.94
&
@target G0.S4
@type xy
1 11.415
&

